SICKLE: A Multi-Sensor Satellite Imagery Dataset Annotated with Multiple Key Cropping Parameters

The availability of well-curated datasets has driven the success of Machine Learning (ML) models. Despite greater access to earth observation data in agriculture, there is a scarcity of curated and labelled datasets, which limits the potential of its use in training ML models for remote sensing (RS) in agriculture. To this end, we introduce a first-of-its-kind dataset called SICKLE, which constitutes a time-series of multi-resolution imagery from 3 distinct satellites: Landsat-8, Sentinel-1 and Sentinel-2. Our dataset constitutes multi-spectral, thermal and microwave sensors during January 2018 - March 2021 period. We construct each temporal sequence by considering the cropping practices followed by farmers primarily engaged in paddy cultivation in the Cauvery Delta region of Tamil Nadu, India; and annotate the corresponding imagery with key cropping parameters at multiple resolutions (i.e. 3m, 10m and 30m). Our dataset comprises 2,370 season-wise samples from 388 unique plots, having an average size of 0.38 acres, for classifying 21 crop types across 4 districts in the Delta, which amounts to approximately 209,000 satellite images. Out of the 2,370 samples, 351 paddy samples from 145 plots are annotated with multiple crop parameters; such as the variety of paddy, its growing season and productivity in terms of per-acre yields. Ours is also one among the first studies that consider the growing season activities pertinent to crop phenology (spans sowing, transplanting and harvesting dates) as parameters of interest. We benchmark SICKLE on three tasks: crop type, crop phenology (sowing, transplanting, harvesting), and yield prediction

==> sections/analysis.tex <==
\section{Analysis of Results}
\label{sec:analysis}
% During the Mid AI4SG Workshop, we proved the hypothesis that High-Resolution (HR) imagery could improve the performance of the downstream task. A plot-level binary crop classification task (paddy/non-paddy) was chosen for this purpose. Thus, we conduct new experiments based on this assumption. But due to the addition of newer field data after the mid-workshop and the unavailability of more HR images from Planet Labs, we did further experiments using only Landsat-8 and Sentinel-2. Instead of Planet Scope, we used Sentinel-1 in the new experiments. While Sentinel-1 cannot provide high-spatiotemporal resolution data, it is rich in complementary information because of its non-optical sensors, i.e. microwave.

The downstream tasks of interest are $(i)$ Crop Type Mapping, $(ii)$ Phenology Date Prediction, and $(iii)$ Crop Yield Prediction. For paddy, the Phenology Date Prediction task is itself composed of $3$ sub-tasks, i.e. sowing, transplanting and harvesting date prediction. % We only present an analytical review of the findings in the main paper. The experimental results are presented in the Appendix section. 
Looking at the results obtained from the conducted experiments, we make the following observations:
\begin{itemize}
% Table \ref{tab:yield-uncommon}
    \item Even though higher spatial resolution data provides more detailed information, spectral resolution plays a vital role in the performance of the tasks. As compared to higher spatial but lower spectral resolution data, a lower spatial resolution along with a higher spectral resolution can improve performance significantly. For example, in Table \ref{tab:yield-uncommon}, a model with all the sensors of L8 (Row \textbf{All}), having 30m spatial resolution, performs better than some of the band combinations of S2 (Rows \textbf{RE3} and \textbf{RE4}), having 10m spatial resolution. 
    % the RGB and NIR band combination of S2 (Table \ref{tab:yield-common}), having 10m spatial resolution, for the yield prediction task. Also, RMSE achieved using all the L8 bands is lower than the RMSE achieved with some of the S2 bands.
    % In the same table, it is also worth noticing that the results obtained using SWIR-1 and SWIR-2 bands alone perform better than the RGB and NIR band combination (maximum spectral resolution of Planet Scope). 
    Thus we hypothesize that with a high spatial and spectral resolution we can achieve even better performance. There exist methods to improve the spectral resolution \cite{rgb2nir, nir-generation} by generating new spectral bands, but these methods need ground truth band values. Recent works on pan-sharpening for improving the spatial resolution are also interesting \cite{pan_comparisons, pan_ICCV, pan_multisensor}; however, these methods are subject to the availability of HR panchromatic bands from the same satellite. An interesting research direction could be to investigate cross-satellite fusion to get high spectral resolution.
    
    \item Since certain spectral bands are more sensitive than others for a given downstream task, naively selecting all the spectral bands does not guarantee better performance. For instance, in Table \ref{tab:yield-common}, some of the band combinations perform better than the results obtained by naively selecting all the band combinations. At the same time, certain combinations downgraded the performance. 
    Therefore, the design of a learning-based algorithm to intelligently select the best band combination depending on the primary task under consideration could be useful. % Unfortunately, to the best of our knowledge, there exists no such method. This is another promising research direction. 
    % Table \ref{tab:yield-fusion}
    \item Using multi-sensor data from multiple satellites improves the performance of the downstream tasks, as shown in Table \ref{tab:yield-fusion}. Even though cross-satellite fusion led to improved performance, it is worth noting that different satellites have varying characteristics, such as pose, orientation, swath width, altitude, sensors and their sensitivity, etc., which may impact accuracy. Our early fusion strategy simply ignores these fundamental differences.  In \cite{MISR-HSI-MSIReview}, the authors report the impact of geo-registration errors on fusion performance. Similarly, solar angles, swath width etc., may also lead to pixel-wise differences between images. %  Unfortunately, the current literature focuses on data-driven learning methods instead of geometry-aware learning.
    \item Employing the actual growing season for Crop Yield Prediction improves the performance significantly in comparison with the usage of the standard growing season.
\end{itemize}
